Federated Action Recognition on Heterogeneous Embedded Devices

Federated learning allows a large number of devices to jointly learn a model without sharing data. In this work, we enable clients with limited computing power to perform action recognition, a computationally heavy task. We first perform model compression at the central server through knowledge distillation on a large dataset. This allows the model to learn complex features and serves as an initialization for model fine-tuning. The fine-tuning is required because the limited data present in smaller datasets is not adequate for action recognition models to learn complex spatio-temporal features. Because the clients present are often heterogeneous in their computing resources, we use an asynchronous federated optimization and we further show a convergence bound. We compare our approach to two baseline approaches: fine-tuning at the central server (no clients) and fine-tuning using (heterogeneous) clients using synchronous federated averaging. We empirically show on a testbed of heterogeneous embedded devices that we can perform action recognition with comparable accuracy to the two baselines above, while our asynchronous learning strategy reduces the training time by 40%, relative to synchronous learning.

==> macros.tex <==
% Use the postscript times font!
\usepackage{times}
\usepackage{soul}
\usepackage{url}
% \usepackage[hidelinks]{hyperref}
% \usepackage[utf8]{inputenc}
\usepackage[small]{caption}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algorithmic}
\urlstyle{same}

% the following package is optional:
%\usepackage{latexsym}

% See https://www.overleaf.com/learn/latex/theorems_and_proofs
% for a nice explanation of how to define new theorems, but keep
% in mind that the amsthm package is already included in this
% template and that you must *not* alter the styling.
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}

% Following comment is from ijcai97-submit.tex:
% The preparation of these files was supported by Schlumberger Palo Alto
% Research, AT\&T Bell Laboratories, and Morgan Kaufmann Publishers.
% Shirley Jowell, of Morgan Kaufmann Publishers, and Peter F.
% Patel-Schneider, of AT\&T Bell Laboratories collaborated on their
% preparation.

% These instructions can be modified and used in other conferences as long
% as credit to the authors and supporting agencies is retained, this notice
% is not changed, and further modification or reuse is not restricted.
% Neither Shirley Jowell nor Peter F. Patel-Schneider can be listed as
% contacts for providing assistance without their prior permission.

% To use for other conferences, change references to files and the
% conference appropriate and use other authors, contacts, publishers, and
% organizations.
% Also change the deadline and address for returning papers and the length and
% page charge instructions.
% Put where the files are available in the appropriate places.

\usepackage{todonotes}
\usepackage[hang,flushmargin]{footmisc} 
% \usepackage[hidelinks,colorlinks=false]{hyperref}
\usepackage{hyperref}
\hypersetup{
    colorlinks=false,
    hidelinks,
}

% Replace this with the name of our system
\newcommand{\name}{{\sc Chorus}\xspace}
\newif\ifdraft
% For final version, replace next line by \draftfalse
\drafttrue %for draft version
% \draftfalse
\newcommand{\saurabh}[1]{\ifdraft{\todo[inline,color=cyan!40]{saurabh: #1}}\fi}
\newcommand{\biplab}[1]{\ifdraft{\todo[inline,color=blue!40]{biplab: #1}}\fi}
\newcommand{\somali}[1]{\ifdraft{\todo[inline,color=red!40]{somali: #1}}\fi}
\newcommand{\pranjal}[1]{\ifdraft{\todo[inline,color=olive!40]{pranjal: #1}}\fi}
\definecolor{coquelicot}{rgb}{1.0, 0.22, 0.0}
\newcommand{\shreyas}[1]{\ifdraft{\todo[inline,color=coquelicot!40]{shreyas: #1}}\fi}
% this command enables to remove a whole part of the text
% from the printout
% to use it just enter
% \remove{
% before the text to be excluded and
% }
% after the text
\newcommand{\remove}[1]{}



==> related-work.tex <==
\section*{Related work reading (Not for inclusion in paper)}
{\bf Federated Learning on the Edge}

\begin{enumerate}

\item Wang, Shiqiang, Tiffany Tuor, Theodoros Salonidis, Kin K. Leung, Christian Makaya, Ting He, and Kevin Chan. "Adaptive federated learning in resource constrained edge computing systems." IEEE Journal on Selected Areas in Communications 37, no. 6 (2019): 1205-1221.

Emerging technologies and applications including Internet of Things, social networking, and crowd-sourcing generate large amounts of data at the network edge. Machine learning models are often built from the collected data, to enable the detection, classification, and prediction of future events. Due to bandwidth, storage, and privacy concerns, it is often impractical to send all the data to a centralized location. In this paper, we consider the problem of learning model parameters from data distributed across multiple edge nodes, without sending raw data to a centralized place. Our focus is on a generic class of machine learning models that are trained using gradient-descent-based approaches. We analyze the convergence bound of distributed gradient descent from a theoretical point of view, based on which we propose a control algorithm that determines the best tradeoff between local update and global parameter aggregation, to minimize the loss function under a given resource budget. The performance of the proposed algorithm is evaluated via extensive experiments with real datasets, both on a networked prototype system and in a larger-scale simulated environment. The experimentation results show that our proposed approach performs near to the optimum with various machine learning models and different data distributions.

\item Lim, Wei Yang Bryan, Nguyen Cong Luong, Dinh Thai Hoang, Yutao Jiao, Ying-Chang Liang, Qiang Yang, Dusit Niyato, and Chunyan Miao. "Federated learning in mobile edge networks: A comprehensive survey." IEEE Communications Surveys \& Tutorials 22, no. 3 (2020): 2031-2063.

In recent years, mobile devices are equipped with increasingly advanced sensing and computing capabilities. Coupled with advancements in Deep Learning (DL), this opens up countless possibilities for meaningful applications, e.g., for medical purposes and in vehicular networks. Traditional cloud-based Machine Learning (ML) approaches require the data to be centralized in a cloud server or data center. However, this results in critical issues related to unacceptable latency and communication inefficiency. To this end, Mobile Edge Computing (MEC) has been proposed to bring intelligence closer to the edge, where data is produced. However, conventional enabling technologies for ML at mobile edge networks still require personal data to be shared with external parties, e.g., edge servers. Recently, in light of increasingly stringent data privacy legislations and growing privacy concerns, the concept of Federated Learning (FL) has been introduced. In FL, end devices use their local data to train an ML model required by the server. The end devices then send the model updates rather than raw data to the server for aggregation. FL can serve as an enabling technology in mobile edge networks since it enables the collaborative training of an ML model and also enables DL for mobile edge network optimization. However, in a large-scale and complex mobile edge network, heterogeneous devices with varying constraints are involved. This raises challenges of communication costs, resource allocation, and privacy and security in the implementation of FL at scale. In this survey, we begin with an introduction to the background and fundamentals of FL. Then, we highlight the aforementioned challenges of FL implementation and review existing solutions. Furthermore, we present the applications of FL for mobile edge network optimization. Finally, we discuss the important challenges and future research directions in FL.

{\large Non peer-reviewed articles}

\item Chen, Yujing, Yue Ning, and Huzefa Rangwala. "Asynchronous online federated learning for edge devices with non-iid data." arXiv preprint arXiv:1911.02134 (2019).

Federated learning (FL) is a machine learning paradigm
where a shared central model is learned across multiple
distributed client devices while the training data remains
on edge devices or local clients. Most prior work on
federated learning uses Federated Averaging (FedAvg) as
an optimization method for training in a synchronized
fashion. This involves independent training at multiple
edge devices with synchronous aggregation steps. However,
the assumptions made by FedAvg are not realistic given
the heterogeneity of devices. In particular, the volume
and distribution of collected data vary in the training
process due to different sampling rates of edge devices.
The edge devices themselves also vary in their available
communication bandwidth and system congurations, such
as memory, processor speed, and power requirements. This
leads to vastly different training times as well as model/data
transfer times. Furthermore, availability issues at edge
devices can lead to a lack of contribution from specific
edge devices to the federated model. In this paper, we
present an Asynchronous Online Federated Learning (ASO-
fed) framework, where the edge devices perform online
learning with continuous streaming local data and a central
server aggregates model parameters from local clients. Our
framework updates the central model in an asynchronous
manner to tackle the challenges associated with both varying
computational loads at heterogeneous edge devices and edge
devices that lag behind or dropout. Experiments on three
real-world datasets show the effectiveness of ASO-fed on
lowering the overall training cost and maintaining good
prediction performance.

\item Xu, Zirui, Zhao Yang, Jinjun Xiong, Jianlei Yang, and Xiang Chen. "Elfish: Resource-aware federated learning on heterogeneous edge devices." arXiv preprint arXiv:1912.01684 (2019).

In this work, we propose ELFISH - a resource-aware federated learning framework to tackle computation stragglers in federated learning. In ELFISH, neural network models' training consumption will be firstly profiled in terms of different computation resources. Guided by profiling, a "soft-training" method is proposed for straggler acceleration, which partially trains the model by masking a particular number of resource-intensive neurons. Rather than generating a deterministically optimized model with diverged structure, different sets of neurons will be dynamically masked every training cycle and will be recovered and updated during parameter aggregation, ensuring comprehensive model updates overtime. The corresponding parameter aggregation scheme is also proposed to balance the contribution from soft-trained models and guarantee the collaborative convergence. Eventually, ELFISH overcomes the computational heterogeneity of edge devices and achieves synchronized collaboration without computational stragglers. Experiments show that ELFISH can provide up to 2x training acceleration with soft-training in various straggler settings. Furthermore, benefited from the proposed parameter aggregation scheme, ELFISH improves the model accuracy for 4\% with even better collaborative convergence robustness. 
\end{enumerate}

{\bf Proofs with knowledge distillation}

\begin{enumerate}
    \item Daniel Hsu, Ziwei Ji, Matus Telgarsky, Lan Wang, "Generalization bounds via distillation," ICLR 2021 (Spotlight).
    
    This paper provides a suite of mathematical tools to bound the generalization error of networks that possess low-complexity distillations --- that is, when there exist simple networks whose softmax outputs approximately match those of the original network.  The primary contribution is the aforementioned bound, which upper bounds the test error of a network by the sum of its training error, the distillation error, and the complexity of the distilled network.  Supporting this, secondary contributions include: a generalization bound which can handle convolutions and skip connections, a generalization analysis of the compression step leading to a bound with small width- and depth-dependence via weight matrix stable ranks, and a sampling theorem to sparsify dense networks.  The bounds and their behavior are illustrated empirically on the standard mnist and cifar datasets.

    
\end{enumerate}

